Renormalization of SU(2) Yang-Mills theory with Flow Equations

We give a proof of perturbative renormalizability of SU(2) Yang--Mills theory in four-dimensional Euclidean space which is based on the Flow Equations of the renormalization group. The main motivation is to present a proof which does not make appear mathematically undefined objects (as for example dimensionally regularized generating functionals), which permits to parametrize the theory in terms of {\it physical} renormalization conditions, and which allows to control the singularities of the correlation functions of the theory in the infrared domain. Thus a large part of the proof is dedicated to bounds on massless correlation functions.

==> pics/junc_gamma1_phi2.tex <==
\begin{picture}(48,16)
%
% lines
\put(0,2){\line(1,0){48}}
%
%vertices
\put(0,2){\circle*{4}}
\put(48,2){\circle*{4}}
%
%labels
\put(-2,8){$\phi_0$}
\put(44,8){$\phi_1$}
\put(23,4){*}
\put(23,-4){$\ubar{\sigma}$}
\end{picture}

==> pics/junc_gamma1_phi3_e.tex <==
\begin{picture}(48,26)
%
% lines
\put(0,2){\line(1,0){48}}
\put(24,2){\line(0,1){24}}
%
%vertices
\put(24,24){\circle*{4}}
\put(0,2){\circle*{4}}
\put(24,2){\circle*{8}}
\put(24,2){\color{white}\circle*{6}}
\put(48,2){\circle*{4}}
%
%labels
\put(27,22){$\phi_0$}
\put(-2,8){$\phi_1$}
\put(44,8){$\phi_2$}
\put(8,4){**}
\put(9,-4){$\ubar{2}$}
\end{picture}

==> pics/junc_gamma_1.tex <==
\begin{picture}(48,26)
%
% lines
\put(0,2){\line(1,0){48}}
\put(24,2){\line(0,1){24}}
%
%vertices
\put(24,24){\circle*{4}}
\put(0,2){\circle*{4}}
\put(24,2){\circle*{8}}
\put(24,2){\color{white}\circle*{6}}
\put(48,2){\circle*{4}}
%
%labels
\put(26,22){$\gamma$}
\end{picture}
